Towards Effective Resource Procurement in MEC: a Resource Re-selling Framework

On-demand and resource reservation pricing models have been widely used in cloud computing, catering to different user requirements. Nevertheless, in Multi-Access Edge Computing (MEC), as the edge has limited resources compared to the cloud, on-demand users may not get their jobs served on time, or at all, if too many resources were reserved by reservation plan users. Concurrently, reservation plan users may possess excess un-utilized quota. To optimize this resource mismatch scenario, we propose a Sharing Quota Model (SQM) where reservation plan users can re-sell unused resource quota to on-demand users, with the mobile network operator (MNO) taking a commission. To analyze the user's aggregate behavior at equilibrium and investigate the MNO's incentive of allowing re-selling, we formulate a 3-stage non-cooperative Stackelberg Game. Solving this game, we characterize the optimal strategies of buyers and re-sellers. We show that on aggregate, users' optimal strategies give rise to 4 disjoint regions, dependent on the MNO's prices and supply levels. Based on this, we characterise the MNO's optimal prices for on-demand users. Numerical results show that having both the sharing and on-demand pool gives the MNO an optimal revenue when the on-demand pool's supply is low, and when the MNO's commission is low.

==> biographies.tex <==
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,keepaspectratio]{Quek_Photo.jpg}}]
{Tony Q.S. Quek}(S'98-M'08-SM'12-F'18) received the B.E.\ and M.E.\ degrees in electrical and electronics engineering from the Tokyo Institute of Technology in 1998 and 2000, respectively, and the Ph.D.\ degree in electrical engineering and computer science from the Massachusetts Institute of Technology in 2008. Currently, he is the Cheng Tsang Man Chair Professor with Singapore University of Technology and Design (SUTD) and ST Engineering Distinguished Professor. He also serves as the Director of the Future Communications R\&D Programme, the Head of ISTD Pillar, and the Deputy Director of the SUTD-ZJU IDEA. His current research topics include wireless communications and networking, network intelligence, non-terrestrial networks, open radio access network, and 6G.

Dr.\ Quek has been actively involved in organizing and chairing sessions, and has served as a member of the Technical Program Committee as well as symposium chairs in a number of international conferences. He is currently serving as an Area Editor for the {\scshape IEEE Transactions on Wireless Communications}. 

Dr.\ Quek was honored with the 2008 Philip Yeo Prize for Outstanding Achievement in Research, the 2012 IEEE William R. Bennett Prize, the 2015 SUTD Outstanding Education Awards -- Excellence in Research, the 2016 IEEE Signal Processing Society Young Author Best Paper Award, the 2017 CTTC Early Achievement Award, the 2017 IEEE ComSoc AP Outstanding Paper Award, the 2020 IEEE Communications Society Young Author Best Paper Award, the 2020 IEEE Stephen O. Rice Prize, the 2020 Nokia Visiting Professor, and the 2022 IEEE Signal Processing Society Best Paper Award. He is a Fellow of IEEE and a Fellow of the Academy of Engineering Singapore.\end{IEEEbiography}

